AI Ethics Education in India: A Syllabus-Level Review of Computing Courses

The pervasive integration of artificial intelligence (AI) across domains such as healthcare, governance, finance, and education has intensified scrutiny of its ethical implications, including algorithmic bias, privacy risks, accountability, and societal impact. While ethics has received growing attention in computer science (CS) education more broadly, the specific pedagogical treatment of {AI ethics} remains under-examined. This study addresses that gap through a large-scale analysis of 3,395 publicly accessible syllabi from CS and allied areas at leading Indian institutions. Among them, only 75 syllabi (2.21%) included any substantive AI ethics content. Three key findings emerged: (1) AI ethics is typically integrated as a minor module within broader technical courses rather than as a standalone course; (2) ethics coverage is often limited to just one or two instructional sessions; and (3) recurring topics include algorithmic fairness, privacy and data governance, transparency, and societal impact. While these themes reflect growing awareness, current curricular practices reveal limited depth and consistency. This work highlights both the progress and the gaps in preparing future technologists to engage meaningfully with the ethical dimensions of AI, and it offers suggestions to strengthen the integration of AI ethics within computing curricula.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conc}

==> findings.tex <==
\section{Findings}
\label{sec:ResultsAndAnalysis}

In describing the overall picture of AI ethics education as presented by this large sample of syllabi, we include descriptions of: (a) who teaches AI ethics, (b) content and duration of instruction, (c) assessments used and (d) learning outcomes in these classes.  

% total%, gender, university ranks, stand alone or embedded, how many hrs
\subsection{Extent of AI Ethics Coverage in Computing Education}

Among the 3395 CS allied courses analyzed, only about 2.21\% (75 courses) included instruction on AI ethics in some form; either as a topic, a module, or an entire course on AI ethics. While this dataset may not represent the full landscape of AI ethics courses across all universities, it reflects a diverse cross-section of institutions. In total, the dataset spans 36 distinct universities (since a number of universities had multiple courses listed). These courses also represent both private (16) and public universities (20), and range from R1 research universities to liberal arts and teaching colleges. Table ~\ref{table:rankRange} shows the QS ranking range where these universities belong. 

%\begin{table}[h]
%\vspace{-0.2cm}
%\caption{\centering Ranking Range of Universities Offering AI Ethics Courses %(N=36)}\label{table:rankRange}
%\vspace{-10pt}
%\centering
 %       \begin{tabular}{rr}
  %      \toprule
   %     \textbf{Rank Range} & \textbf{Frequency} 
    %    \\ \midrule
     %   1 to 50 & 13 \\
      %  51 to 100 & 9 \\
       % 101 to 200 & 0 \\
        %201 to 500 & 11\\
        %Above 500 & 3\\
        %\hline
        %\end{tabular}    
%\end{table}

The 75 courses that included AI ethics were taught by 75 unique instructors. Our analysis also showed a relatively balanced distribution of faculty across academic ranks: 16\% were assistant professors, 12.5\% associate professors, and 22\% full professors. The remaining instructors were composed of adjunct faculty, lecturers, research scientists, and other non-tenure-track positions.

In terms of instructional approach, AI ethics was integrated into the curriculum in two primary ways: as a standalone course or embedded within broader technical courses. Figure~\ref{fig:coverage} illustrates the extent of AI ethics coverage across the analyzed syllabi. As shown, the majority of courses (~59\%) addressed AI ethics in a single session, with around 15.7\% covering the topic over the span of a week (defined here as 3 to 5 sessions). Additionally, 13.3\% of courses included AI ethics in two sessions, while 12\% were dedicated entirely to the subject.

Examples of dedicated course titles include Intelligent Systems: Design and Ethical Challenges, Artificial Intelligence Ethics, Responsible AI in Societal Deployment, and AI Ethics in Social Impact. In contrast, many courses embedded AI ethics technical subjects such as Fundamentals of AI, Machine Learning, Deep Learning, Natural Language Processing, Reinforcement Learning, AI System Design, Applied or Advanced Machine Learning, Generative AI, Trustworthy Machine Learning, Human-Centered AI, Intelligence for Robotics, Human-Computer Interaction, and Data Science.

\begin{figure}[h]
    \centering
    \resizebox{0.35\textwidth}{!}{%
    \begin{tikzpicture}
        \pie[text=pin, color={
                blue!30,    % Light blue for One Session
                green!30,  % Light green for One Week
                orange!30, % Light orange for Two Sessions
                red!30    % Light red for Complete Course
            }]
        {59.04/ One Session on AI Ethics, 15.66/ One Week of AI Ethics, 13.25/Two Sessions on AI ethics, 12.05/Complete course on AI Ethics}
    \end{tikzpicture}%
    }
    \caption{AI Ethics Coverage from Syllabi Analysis (N=83)}
    \label{fig:coverage}
    \vspace{-2mm}
\end{figure}

While dedicated courses typically included more than 15 hours of AI ethics content, the majority of embedded courses (78\%) addressed AI ethics for only 0 to 5 hours, with the remaining covering between 5 and 10 hours. Notably, approximately 4\% of all courses incorporated guest lectures to address AI ethics topics, offering an alternative approach to integrating ethical perspectives.  We also examined the academic level at which the courses were offered. Of the courses analyzed, 92\% were taught at the undergraduate level, 6\% at the graduate level, and 2\% were cross-listed for both. Among the undergraduate courses, approximately 60\% appeared to be upper-division (junior/senior level) based on course number, title, description, and prerequisites, while the remaining 40\% were lower-division (freshman/sophomore 
level).

\subsection{Topics part of AI Ethics Education}

The qualitative analysis of 83 course syllabi led to a diverse set of themes or topics covered in AI ethics (Table ~\ref{table:topicsAIEthics})\footnote{Note that the sum need not be 100\% as few topics are covered in multiple courses)}. The most frequently addressed topic is \textbf{algorithmic bias and fairness} in intelligent systems, covered in 38\% of courses. These topics introduce students to methods for detecting bias in data and model outputs, highlighting how social inequalities can be encoded and amplified by machine learning systems. Many syllabi include formal definitions and fairness metrics—such as demographic parity and equalized odds—and explore the trade-offs these present in practice. Several courses go further by covering algorithmic debiasing techniques, including reweighting, adversarial learning, and post-processing strategies, often grounded in real-world case studies. The ethical implications of biased systems are also emphasized, particularly in high-stakes applications such as hiring, healthcare, and criminal justice. Some courses contextualize fairness within broader frameworks of social justice, examining how equity and inclusion can inform the design and evaluation of AI systems. Additionally, fairness is explored in domain-specific contexts—for example, in NLP through biased language generation and content moderation, or in healthcare via clinical risk models and diagnostic tools.

\begin{table}[h]
\vspace{-0.2cm}
\caption{\centering Topics covered in AI Ethics (N=83)}\label{table:topicsAIEthics}
\vspace{-10pt}
\centering
        \begin{tabular}{lr}
        \toprule
        \textbf{Theme/Topic} & \textbf{Coverage} 
        \\ \midrule
      Algorithmic Bias and Fairness & 38\% \\
      Transparency and Explainability & 31\% \\
      Privacy and Data Governance & 29\% \\ 
      Social Impact and Justice & 27\% \\ 
      AI Safety and Robustness & 26\% \\
      Human-AI Interaction and Agency & 24\% \\
      Ethical Frameworks and Moral Reasoning & 21\% \\
      Accountability and Policies & 19\% \\
      Generative AI specific concerns & 18\% \\
      Environment and Labor related & 12\% \\
        \hline
        \end{tabular} \vspace{-6pt}
\end{table}

\textbf{Transparency and explainability} is the next most common theme, featured in 31\% of courses. These courses emphasize the need for interpretable AI systems, exploring techniques like rule extraction, saliency maps, and model inspection to make AI decisions understandable to users and stakeholders. A few courses also explore how interpretability applies to large language models and foundation models, highlighting evaluation and benchmarking practices. Some syllabi address the limitations and trade-offs of explainability, encouraging students to critically assess when and how transparency can be achieved in practice.

\textbf{Privacy and data governance}, covered by 29\% of courses, dealt with responsible data use, anonymization, and compliance with privacy frameworks. In addition to general privacy principles, several courses explored specific concerns such as privacy risks in generative AI and large language models, including issues like prompt injection attacks, demographic inference, and watermarking techniques. Other topics included algorithmic approaches for protecting personal traits from being reverse-engineered and discussions around the ethical use of clinical data in healthcare machine learning systems. Some courses also addressed broader policy and legal frameworks, referencing governance mechanisms such as the EU AI Act and U.S. Senate proposals for regulating AI privacy.

Courses also address topics around \textbf{social impact and justice} (27\%), focusing on how AI technologies influence domains such as healthcare, education, law enforcement, and employment. These courses encourage students to consider the equity implications of AI deployment, especially on marginalized communities. Specific topics include the role of AI in predictive policing, HIV and tuberculosis prevention, and public safety, as well as understanding systemic inequities embedded in data-driven decision systems. Some courses integrate frameworks of justice, rights, and welfare into machine learning curricula and emphasize participatory or interdisciplinary design involving experts from social work, criminology, and public health. Closely related is the topic of \textbf{AI safety and robustness} (26\%), which focuses on reliability, adversarial robustness, and secure system behavior in real-world settings. Topics covered include adversarial robustness, uncertainty quantification, and safe reinforcement learning, as well as emerging risks posed by generative AI and large language models. %Courses explore attack vectors like prompt injection and model misuse, as well as safety alignment strategies such as human-in-the-loop training, trojan detection, and model unlearning. 
Some courses contextualize safety within broader societal implications—such as preventing harm from autonomous systems in healthcare or transportation—and discuss the importance of aligning AI behavior with human intent.

Courses addressing the theme of \textbf{human-AI interaction and agency} (24\%) focus on how AI systems can be designed to support meaningful, ethical, and effective collaboration between humans and machines. Topics include human-centered design principles, user interface strategies for AI-driven systems, and methods for enabling human-AI teaming and interpretability. These courses explore how to design interactive, human-in-the-loop systems—particularly in the context of large language models—while emphasizing the importance of preserving human agency and trust. Meanwhile, \textbf{ethical frameworks and moral reasoning} are covered in 21\% of the courses, introducing students to philosophical approaches such as utilitarianism, deontology, and virtue ethics, and equipping them to reason through complex dilemmas posed by intelligent systems. These frameworks are applied to AI-related moral dilemmas, helping students develop skills in ethical reasoning and decision-making. Topics include ethical considerations in digital technologies, IRB-style human subjects research ethics, and real-world case studies that challenge students to connect theoretical concepts with contemporary AI issues.

More specialized but still significant themes include \textbf{accountability and policy} (19\%), which explores questions of responsibility in AI system failures and oversight structures. Courses addressing this theme cover topics such as responsible AI deployment, democratized governance, and the integration of ethical principles into policy frameworks, often illustrated through case studies in healthcare, education, and employment. \textbf{Generative AI-specific concerns}—including misinformation, value misalignment, and prompt injection—appear in 18\% of courses. Courses also engage with the societal implications of generative AI, including misinformation, content moderation, and regulatory challenges. Finally, \textbf{environmental and labor ethics}, covered in 12\% of the syllabi, address the hidden costs of AI, highlighting the energy demands of training large models and the often-overlooked labor involved in data labeling and content moderation. Some courses discuss sustainable system design and advocate for ethical awareness of the ecological and human toll of AI development.

\subsubsection{Resources used to teach AI Ethics}
We examined the syllabi for references to AI ethics-specific resources or textbooks. The majority of the courses (over 90\%) did not include any dedicated materials for teaching AI ethics in the syllabus. Instead, they primarily included standard AI and machine learning textbooks—such as Artificial Intelligence: A Modern Approach\cite{10.5555/1671238} by\citeauthor{10.5555/1671238}, Pattern Recognition and Machine Learning\cite{10.5555/1162264} by ~\citeauthor{10.5555/1162264}, and other widely used texts aligned with the technical focus of the core course in which AI ethics content was embedded. Only a small number of syllabi explicitly mentioned ethics-specific resources, such as AI for Social Impact \footnote{\url{https://ai4sibook.org/}}, Fairness and Machine Learning: Limitations and Opportunities\cite{barocas-hardt-narayanan}, The Ethical Algorithm: The Science of Socially Aware Algorithm Design\cite{10.5555/3379082}, The Alignment Problem: Machine Learning and Human Values\cite{christian2021alignment}, Artificial Intelligence: A Guide for Thinking Humans\cite{mitchell2019ai}, and Human Compatible: Artificial Intelligence and the Problem of Control~\cite{russell2019human}.

% LO, assessment, when it's taught
\subsection{Learning Objectives (LO) in AI Ethics Education}
This section presents the learning objectives (LO), assessment methods found from the analysis. 

\subsubsection{Learning Objectives}
The terms “learning objectives” and “learning outcomes” have subtle differences in meaning but are often used interchangeably~\cite{Harden01012002}; we saw both in our data. Similar to a 2020 syllabus analysis published in SIGCSE on tech ethics~\cite{fiesler_what_2020}, we use the term \textit{learning outcome} to mean an explicit statement of what students should know or be able to do by the end of the course related to AI ethics, regardless of how such a statement might be labeled in any given syllabus. Our qualitative coding revealed eight common types of learning outcomes in terms of what students should be able to do by the end of the course.
\begin{enumerate}[leftmargin=*]
    \item Identify and evaluate privacy risks in AI systems, and propose strategies to mitigate them within ethical and legal frameworks
    \item Detect, analyze, and correct algorithmic biases in datasets and models to promote fairness in AI applications
    \item Interpret and communicate the decision-making processes of AI systems using explainability techniques
    \item Discuss or Critique key ethical dilemmas encountered during the design, training, and deployment choices of AI systems
    \item Seeing multiple perspectives of AI technologies and their impact on democratic processes, civil liberties, and human rights across societal contexts
    \item Investigate and compare ethical frameworks, regulatory strategies, and policy approaches relevant to AI governance
    \item Apply ethical reasoning models to assess and justify decisions made in the development and deployment of AI systems
    \item Considering the consequences of unethical AI system design and creating solutions with an emphasis on user agency, transparency, and trust
\end{enumerate}

\subsubsection{Assessment Methods}
The majority of courses did not include any documented assessments specifically focused on AI ethics topics. Only 18\% of syllabi indicated the use of quizzes to evaluate student understanding of ethical concepts. A smaller proportion—approximately 5\%—incorporated more reflective or discussion-based methods, such as group reflections, case studies, and assignments, as part of their AI ethics assessment strategies. A few dedicated AI ethics courses outlined more structured evaluation formats, including activities like a "Statement of Interest," where students were asked to articulate the importance of a particular ethical aspect of trustworthy AI and identify a relevant application area. Other assignments included paper critiques that required students to evaluate the strengths and weaknesses of a current method from an ethical lens, along with written homework assignments and graded class participation or discussions. While it is possible that written exam questions addressing AI ethics may be included in broader course assessments, such details were typically not documented in the syllabi reviewed. Overall, these findings suggest that assessment of AI ethics remains limited and inconsistently integrated across computing curricula.
